Human Motion Control of Quadrupedal Robots using Deep Reinforcement Learning

A motion-based control interface promises flexible robot operations in dangerous environments by combining user intuitions with the robot's motor capabilities. However, designing a motion interface for non-humanoid robots, such as quadrupeds or hexapods, is not straightforward because different dynamics and control strategies govern their movements. We propose a novel motion control system that allows a human user to operate various motor tasks seamlessly on a quadrupedal robot. We first retarget the captured human motion into the corresponding robot motion with proper semantics using supervised learning and post-processing techniques. Then we apply the motion imitation learning with curriculum learning to develop a control policy that can track the given retargeted reference. We further improve the performance of both motion retargeting and motion imitation by training a set of experts. As we demonstrate, a user can execute various motor tasks using our system, including standing, sitting, tilting, manipulating, walking, and turning, on simulated and real quadrupeds. We also conduct a set of studies to analyze the performance gain induced by each component.

==> sec/backup_Learning.tex <==
\section{Motion Imitation}
- The next step is to develop a control policy that allows the robot to imitate the given retargeted motion.
- 

Our framework aims to obtain a solid controller that enables the robot to perform a wide range of motor skills interactively. To generate the variously changing target control decision in a short time, we deploy reinforcement learning(RL) which automatically acquires the motor skills with a short computation time. However, learning the policy for real-world tasks from scratch involves critical challenges such as the consumption of a long learning time and possible hardware damage. To avoid the challenges caused by learning in the real world, we build a physically simulated environment from the Raisim simulator~\cite{raisim} that approximates a real-world physics system. From the simulated environment, an agent learns the policy much faster by high computing power without any hardware damage. The learned policy is then transferred to the real world domain by domain adaptation technique. 
\par
% Learning from imitation reward 
As stated in the mapper section, our framework generates the kinematic motion from the mapping of the human motion. Therefore, a robot should imitate the mapped motion while following the physics law. We formulate imitating a mapped motion as a reinforcement learning goal inspired by previous studies[cite many]. To guarantee controllability for any human motion input, the policy should be learned with all possible mapped motions. The simple method to solve this problem is learning a single policy to cover all reference motions mapped from all plausible human motions. This method faces two challenges: learning all motion in one policy and providing all range of plausible human motion for reference mapping. First, learning all possible motions at once often leads to learning failure due to the complexity of building different strategies for all possible tasks. However, training policies motion by motion is practically impossible due to limited resources. We trained a single policy for a single mapping state mentioned in Section XXX. A policy is capable of learning various motor skills within the same mapping state since the states are classified by balancing strategy which plays a critical role in adapting to a physics environment. Second, we need to design and solve an optimization problem that generates plausible task-oriented motion with a random variable to deliver human motion input for generating reference motions. This process involves high manual work defining tasks and constraints and time-consuming computation solving the problem. To overcome this challenge, our system generates reference motion directly by motion generator used for data preparation of mapper. The assumption for this decision is that the out motions from the mapper might not much different from the motions from the generator used for training data preparation. At beginning of each training episode, the system generates reference motion from the generator using random vector $\alpha$. As this motion is constrained to a generator function, the noise vector $\vc{n}$ is injected to obtain a wider range of motion possibly generated by the mapper. 
\subsection{Reinforcement Learning for a Single Task}
%General Formulation
In RL, an agent interacts with an environment, aiming to learn an optimal policy $\pi$ that provides the maximum of its expected return for a given task. At each time step $t$, the agent utilizes the observed state $\vc{s}_{t}$ as an input to sample an action $\vc{a}_{t} \sim \pi(\vc{a}_{t} | \vc{s}_{t})$ from its policy $\pi$. The action $\vc{a}_{t}$ is then applied to the agent, resulting a new state $\vc{s}_{t+1}$ and a scalar reward $r_t = r( \vc{s}_{t},\vc{a}_{t},  \vc{s}_{t+1})$. The expected return $J(\pi)$ which a policy aim to maximize is defined from the trajectory $\tau = \{( \vc{s}_{0},\vc{a}_{0},  \vc{s}_{1}), ( \vc{s}_{1},\vc{a}_{1},  \vc{s}_{2}), \cdots \}$ cummulated by repeated process. The $J(\pi)$ is defined as below equation with time horizon of each episode $T$ and discount factor $\gamma \in [0,1)$ driving the return to be finite. 
\begin{equation}
J(\pi) = \set{E}_{r \sim p(r|\pi)}[\sum_{t=0}^{T-1} \gamma^{t} r_{t}]
\label{eq:expected return}
\end{equation}
Probability $p(r|\pi)$ represents the likelihood of a trajectory $\tau$ under a given policy $\pi$ since RL assumes the Markov property of probability in transition probability. 
\begin{equation}
p(r|\pi) = p(\vc{s}_{0}) \prod_{t=0}^{T-1} p(\vc{s}_{t+1}|\vc{s}_{t}, \vc{a}_{t}) \pi(\vc{a}_{t}|\vc{s}_{t})
\label{eq:transition probability}
\end{equation}
where as $p(\vc{s}_{0})$ denotes the initail state distribution and $p(\vc{s}_{t+1}|\vc{s}_{t}, \vc{a}_{t})$ denotes the state transition probability which in our case, the dynamics of the simulation environment. 
\par
%Detailed Formulation
We start our RL design from assigning a single task for one policy. In our design of RL, an agent augments the input of policy $\pi$ from the observed state $\vc{s}_{t}$ and the goal reference motion from the mapper  $\vc{g}_{t}$ to sample the action $\vc{a}$ over distribution $\pi(\vc{a}_{t} | \vc{s}_{t}, \vc{g}_{t})$. The state $\vc{s}_{t} = (\vc{p}_{t-3:t}, \vc{a}^{f}_{t-3: t-1})$ observes history of the robot $\vc{p}_{t-3:t}$ pose feat and the filtered action history $\vc{a}^{f}_{t-3: t-1}$ in the four and three timesteps respectively. The robot pose features $\vc{p}_{t}$ consist of the readable features from the real robot: root orientation and the local rotation of every joint. The root orientation is sensored by IMU readings and converted to quaternion for consisting a pose features. A goal $\vc{g}_{t} = \vc{\hat{p}}_{t-3:t}$ is defined as history of reference poses to imitate. The previous study [cite] explicity provides future reference poses to accelerate the learning but our system view the history since our system takes on-line target reference motion mapped from the human motion that is unpredictable. The action $\vc{a}_{t}$ defines as the PD target for the twelve joint motors of a robot. To generate the smoother motions, the action is passed through the low-pass filter to generate $\vc{a}^{f}_{t}$ which is actually applied on the robot and the state description.
\par
\noindent \textbf{Reward function } The design of rewards for each task shares a similar framework but varies in detail. The base of the reward function encourages the agent to imitate the given reference motion while adapting to the physics simulation. The base of the reward at each time step t is designed as:
\begin{equation}
r_t = w^{main}r_{t}^{p} \cdot r_{t}^{e} \cdot r_{t}^{rp} \cdot r_{t}^{ro} \cdot r_{t}^{sp}  + w^{acc}r_{t}^{acc} 
\label{eq:base reward function design}
\end{equation}
$$
w^{main} = 0.9, w^{acc} = 0.1
$$
The main reward terms are combined by multiplication inspired by previous works~\cite{lee_2019_rl, park_2019_rl}. The terms bound with multiplication are forced to be non-zero to convey reasonable meaning for every component. Each reward term is designed as follows:
\begin{equation}
    r_{t}^{p} =  \exp{(s_{p}\sum_j \norm{\hat{\vc{p}}_{t}^{j} - \vc{p}_{t}^{j}}^2)}
\label{eq:pose reward function design}
\end{equation}
$r_{t}^{p}$ refers to a joint imitation reward. This term aims to minimize the joint angle difference from the reference position. $r_{t}^{p}$ is defined as below while $\hat{\vc{p}}_{t}^{j}$ represents the joint angle of joint $j$ of the reference motion, $\vc{p}_{t}^{j}$ represents the agent robot's joint. 
\begin{equation}
    r_{t}^{e} =  \exp{(s_{e}\sum_j \norm{\hat{\vc{x}}_{t}- \vc{x}_{t}}^2)}
\end{equation}
The end-effector reward $r_{t}^{e}$ drives the robot to track the end-effector of the reference. $ \vc{x}_{t}$ denotes the 3D position of the end-effector with respect to the root as stated above. 
\begin{equation}
\begin{split}
    r_{t}^{rp} &=  \exp (s_{rp} \norm{\hat{\vc{x}}_{t}^\text{root}- \vc{x}_{t}^\text{root}}^2) \\ 
    r_{t}^{ro} &=  \exp (s_{ro}\lVert \arccos (2<\vc{\hat{p}}^\text{root}_{t}, \vc{p}^\text{root}_{t}>^{2} - 1)\rVert^2) 
\end{split}
\end{equation}
The root position reward $r_{t}^{rp}$ encourages the agent to tract the root 3D position and the root orientation reward $r_{t}^{ro}$ drives the agent to minimize the angle between root orientations expressed in quaternion. 
\begin{equation}
    r_{t}^{sp} =  \exp{(s_{sp}\sum_c \text{DistCSP}(c)^2)}
\end{equation}
\begin{equation}
  \text{DistCSP}(c)=\left\{
  \begin{array}{@{}ll@{}}
    0, & \text{if}\ \text{Inside}(\text{CSP},c) \\
    \text{minDist}(\text{CSP},c), & \text{otherwise}
  \end{array}\right.
\end{equation} 
The support polygon reward $ r_{t}^{sp}$ is only activated when learning the manipulation task in the standing state otherwise, $ r_{t}^{sp} = 1$. When manipulating one leg in the standing state, only three legs support the weight of the robot causing unstable balancing. To stabilize the robot balancing during the manipulation task, we define the support polygon reward that forces to put the balancing components of the robot $c$ - the center of mass(COM), the divergent component of motion(DCM) and the center of pressure(COP) - inside the conservative support polygon(CSP). The CSP is defined as a reduced area of support polygon that shares the same center with the original polygon. Forcing balancing components to be inside the CSP guarantees stable balancing with an external perturbation. Function \text{DistCSP} outputs the distance of balancing component $c$ from the CSP. It returns 0 when $c$ is inside the CSP and the minimum distance from the CSP sides when it is outside.
\begin{equation}
    r_{t}^{acc}=  \exp{(-3.0\sum_j \norm{\ddot{\vc{p}}_{t}}^2)}
\end{equation}
The acceleration reward $r_{t}^{acc}$ which is added to the main reward aims to reduce the shaky movement of the action by minimizing the joint acceleration. Since it plays a supporting role in learning, the reward is added to take 10$\%$ of the total amount of reward while the main reward takes 90$\%$.
\par
% Write the changing scaling. 
The scaling coefficient $s$ for each reward term determines the weight of the reward considered. As $s$ goes larger, the reward term takes the dominant role. We use these properties to emphasize the important factors to be learned during the learning the curriculum which will be introduced at below section.
\par
\textbf{Early termination } The early termination accelerates the learning speed which is proven by many researches[cite]. To escape from unexpected movement, the learning system triggers the early termination when the trunk of the robot touches the ground (falling) and self penetrating contact happens(self-colliding motion). 

\subsection{Curriculum Learning}
The parts of the challenges remain still despite the design of policy for a single task. The first remaining challenge is local optimum behaviour when providing a large range of motion to mimic from the beginning of training. The local optimum policy does not follow the target reactively. Instead, it tries to stuck in a steady position to escape from the early termination and takes small rewards from not falling. The second unsolved challenge is that a policy should cover the whole possible motion for each mapping state. The above policy formulation is limited to controlling the reference for a single task. We introduce a double curriculum during the learning to overcome these challenges: expanding range curriculum to obtain optimal behaviour and then expanding task curriculum to obtain a single policy for a single mapping state which contains multiple tasks.
\par
\noindent \textbf{Motion range curriculum } 
Training a wide range of motion from the beginning of training leads the notoriously unstable states to train that cause trapping in a local optimum or even failing to learn the appropriate policy. To solve this issue, the agent learns the curriculum of the given tasks from easy to complicated reference motions. Easy reference motion means the representative motion for a given task with low movement involved. In this manner, the agent first learns the representative motor skills for a given task. Then the complicated motions which the variety of task motion changing agile are given with a certain amount of epoch passed. In addition the scaling coefficients of reward function change over the curriculum. This technique is useful since learning a value function is much faster than learning a policy done within a few epochs. At first, scaling coefficients of joint imitation is set high to powerfully drive the agent to mimic the reference motion. However, after plenty of learning passed, task-related scaling coefficients such as CSP reward in the manipulation task, orientation reward in the tilting task are set high to satisfy the desired intention of human mapping rather than just following the reference motion. 
\par
\noindent \textbf{Task curriculum  } For the same reason with training a wide range of motion from the beginning, training motion for multiple tasks from scratch often leads to failure. This is the reason for training a single task for a policy first. We set the hierarchy of learning for control similar to generating the mapping for multiple tasks in a single state. In the example of the standing state, the agent first learns a policy for any motion transition of tilting task. Then, it passes through the second learning curriculum, manipulating one leg while tilting its body. Learning the multiple tasks curriculum also has a sub-curriculum of expanding range curriculum. Since the policy already learns the optimal policy for the base task, the sub-curriculum of expanding task curriculum provides an easy-to-complicated curriculum for the newly added task and a complicated task for a trained task.

\begin{table}[]
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
\rowcolor[HTML]{C0C0C0} 
\textbf{Parameters}          & \textbf{Range}         & \textbf{Unit} \\ \hline
\\[-1em]
Link Mass                    & [0.75, 1.25] X default & kg           \\ \hline 
\\[-1em]
Ground Friction Coefficients & [0.5, 1.5]             & 1             \\ \hline
\\[-1em]
Proportional Gain                       & [0.7, 1.3] X default   & N/rad           \\ \hline
\\[-1em]
Derivative Gain                       & [0.7, 1.3] X default   & N$\cdot$s/rad       \\ \hline
\\[-1em]
Communication Delay          & [0, 0.016]             & sec           \\ \hline
\\[-1em]
Ground Slope                 & [0, 0.14]             & rad           \\ \hline
\end{tabular}%
}
\label{Tab:Domain Randomization parameters}
\caption{Dynamic parameters and their range for domain randomization}
\end{table}

\subsection{Domain Adaptation}
The gap between the dynamics of the simulation and the real world decreases the performance of policies trained in simulation that are deployed on a real physics system. The domain randomization during training enhances the robustness when applying policy to the real world[cite]. The randomization component generates the uncertainty of the dynamics properties, providing a feasible real-world environment to the agent during the training. Specifically, the randomization increases the variant of the sensor noise and modelling uncertainty that possibly occurs while modeling the simulation environment. The dynamics properties are parameterized as a vector $\vec{\mu}$, whose values are varied between the ranges specified in Table XXX. We also build a curriculum for randomization regiment for policy to gradually adapt to the environments with various dynamics. 

==> sec/backup_Mapping.tex <==
\section{Hetero-morphological Motion Mapping}

% Overview definition of our problem. What is our problem? What is so special?
The first component of our motion-based control system is a hetero-morphological motion mapping module, which converts the user's motion into the corresponding robot motion. Many prior works have demonstrated successful human-to-humanoid motion mapping [cite]. However, a unique challenge of our problem is to infer a mapping function between two different morphologies without leveraging explicit hand-engineered motion features, such as contact states or centroidal dynamics: note that a human and a quadrupedal are governed by very different dynamics and control strategies. Our problem becomes even more challenging with additional issues, such as the sparsity of the data and the required interactivity.

% Our approach (vs. IK, vs. pure NN). Strength of our approach?
We tackle this problem using a hybrid approach that combines [name of the approach, cite] and optimization-based post-processing. Traditional techniques [cite] typically approach motion retargeting by formulating the problem as an optimization problem, but they tend to show a slow turnaround time that is not suitable for interactive applications. And they also often require task-specific formulation, which makes the system hard to handle a wide variety of motions. On the other hand, learning-based approaches showed impressive inference capabilities at interactive rates, but they are known to be data-hungry. In addition, they can also generate inconsistent or unexpected motions that can cause severe damage to the robot. To this end, we propose a hybrid motion mapper module that first infers the motion in a supervised learning fashion from a sparse dataset and corrects the potential inconsistency using optimization at the post-processing stage. This approach allows us to build a fast and robust motion mapper that can be applied to various motor tasks.
\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{fig/FullMapper.png}
\caption{Full mapping diagram}
\end{figure}
% Preview
In the following sections, we first explain how to create a motion mapper for a single task with a limited dataset. Then we will explain how to combine the constructed motion mappers into a single motion mapper using the hierarchical formulation, which allows us to develop accurate mappers in a scalable fashion.
\sunwoo{State machine + hierarchy}

\subsection{Motion Mapper Design for a Single Task}

\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{fig/SingleMapper.png}
\caption{Motion mapper for a single task}
\end{figure}
In this section, we will define the problem of motion mapping and provide the details of our algorithm. In our formulation, a motion mapper $f$ takes a human pose $\vc{q}$ as inputs and maps it into the corresponding robot pose $\vc{p}$. However, a simple pose-to-pose mapping can be ambiguous in periodic motions because a single pose does not contain any temporal information. For instance, we can interpret the same pose in an in-place marching motion as two different phases of swing up or swing down which can be mapped to different robot poses. Therefore, our model learns to map a triplet of the human pose, velocity, and acceleration $(\vc{q}, \vc{\dot{q}}, \vc{\ddot{q}})$ to those of robots $(\vc{p}, \vc{\dot{p}}, \vc{\ddot{p}})$. We estimate the derivatives using finite differences with $\Delta t = 0.1$.

% However, a simple pose-to-pose mapping can be ambiguous in periodic motions because a single pose does not contain any temporal information. For instance, we can interpret the same pose in an in-place marching motion as two different phases of swing up or swing down. In contrast, the corresponding postures of quadrupedal robots have clearly different poses. 

\noindent \textbf{Data Preparation.}
We prepare the dataset $\mathcal{D}$ by collecting matching pairs of human and robot motions. First, we generate robot motions for sampled tasks. For example, tilting or manipulation tasks are synthesized by generating random goals and solving robot poses using inverse kinematics. Then we interpolate these key poses with a random time interval ranging from $1$ to $3$ seconds. For locomotion tasks, we generate a set of walking motions with various speeds and turning rates using deep reinforcement learning, which is similar to the work of [cite]. Please refer to the appendix for the detailed procedure of robot motion generation. Also, please note that the generated motions are used for control policy training in Section XXX.

Once we have the robot motions, we collect the matching human motion sequences. We ask a human user to act the ``corresponding motions'' based on the user's own intuition and capture the motions using a motion capture system. Please note that human motions may be very different from robot motions while a user is trying to maintain the semantics of the robot motion as much as possible. We further manually process the motions to clean up noisy segments and fix asynchronous actions based on contact flags.
\sehoon{Sunwoo, please read this data preparation part and update it if anything is far from what you did. I tried but am not sure.}

% We utilized the motion generators for two uses: generating robot motion for mapper training sets and providing reference motion for the reinforcement learning policy. Each motion generator is assigned to produce each task. The generating vector, $\vec{\alpha}$ which is also varied by the desired tasks decides the kinematic poses to generate. For example, the generating vector for tilting task $\vec{\alpha} = {a_{x}, a_{y}, a_{z}}$ which $a_{i}$ indicates the tilting angle for axis $i$. From decided $\vec{\alpha}$, the tilting motion generator solves the inverse kinematics(IK) to obtain the result robot pose. Likewise, the motion for each goal is determined by the generating vector. See the appendix for detailed generating vector formulation and motion generator function structure. The generated poses with noise injection are also used to feed for training the control policy. A detailed explanation related to it is written in the section V-A. \sehoon{merged with human data generation}



\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{fig/TrainingMapper.png}
\caption{Training mapping using sparse dataset}
\end{figure}
% \sunwoo{I think we need to separate the motion mapper and contact probability training diagram or discard this diagram.}
% Therefore, we extend our mapping problem by considering a short history of states with $\Delta t = 0.1$. We set the number of history $n_h$ to be three, which is sufficient to encode velocity and acceleration while being concise. Therefore, our mapping function $f$ and the dataset $\mathcal{D}$ maps a triplet of human poses $\vc{q}_{t}$, $\vc{q}_{t-1}$, and $\vc{q}_{t-2}$ into a triplet of robot poses $\vc{p}_{t}$, $\vc{p}_{t-1}$, and $\vc{p}_{t-2}$. Although our mapping outputs three robot poses, we only use the most recent pose $\vc{p}_t$ that corresponds to the current human pose $\vc{q}_t$.

\noindent \textbf{Supervised Learning.}
We use multi-layer perceptron (MLP) for training a mapper from the given dataset $\mathcal{D}$. Our MLP consists of three leaky ReLU layers and one final hyperbolic tangent layer. Since a hyperbolic tangent function outputs the value between [-1, 1],  we shift and scale the outputs using the robot joint limit vector to finalize the joint angle of the robot. Our loss function is defined as follows:
\begin{equation}
	L_{map} = w_{ori} L_{ori} + w_{jnt} L_{jnt} + w_{dx} L_{dx} + w_{ddx} L_{ddx},
\end{equation}
where $L_{ori}$ and $L_{jnt}$ measure the differences in the root orientation and joint angles while $L_{dx}$ and $L_{ddx}$ penalizes the differences in the end-effector velocities and accelerations. We omit the function arguments $\vc{p}, \vc{\dot{p}}$, $\vc{\ddot{p}}$, $\vc{\bar{p}}, \vc{\bar{\dot{p}}}$, and $\vc{\bar{\ddot{p}}}$ for brevity, where the former three are the outputs from the networks and the latter three are the target values. More specifically, the orientation loss $L_{ori} = d(\vc{p}^{root}, \vc{\bar{p}}^{root})$ compares the root orientation $\vc{p}^{root}$ in quaternion and its target value $\vc{\bar{p}}^{root}$ via a quaternion distance function $d$. The joint angle loss $L_{jnt}= |\vc{p}^{jnt} - \vc{\bar{p}}^{jnt}|^2$ is designed to match the joint angles $\vc{p}^{jnt}$ and their target values $\vc{\bar{p}}^{jnt}$. Two end-effector terms, $L_{dx} = |\vc{\dot{x}} - \vc{\bar{\dot{x}}}|^2$ and $L_{ddx} = |\vc{\ddot{x}} - \vc{\bar{\ddot{x}}}|^2$ compares the end effector velocities $\vc{\dot{x}}$ and accelerations $\vc{\ddot{x}}$ against their target values, $\vc{\bar{\dot{x}}}$ and $\vc{\bar{\ddot{x}}}$, respectively. Please note that these values can be derived from $\vc{\dot{p}}$ and $\vc{\ddot{p}}$.

% The position loss is designed to minimize the joint angle difference with $\vc{q}_{t}$ being a joint angle of the robot.
% \begin{equation}
% 	L_{p} = w_{p} \lVert \vc{\Bar{p}}_{t}- \vc{p}_{t}\rVert^2 
% \label{eq:joint_angle_loss_function}
% \end{equation}
% The temporal loss components minimize the velocity and acceleration difference of relative 3D position of end-effectors with respect to the root. The idea is that as primary terms try to mimic the kinematic joint poses, the temporal jointly consider the world temporality. As $\vc{x}^{\text{e}}$ denotes the relative 3D positions of end-effectors, $\vc{\dot{x}}^{\text{e}}_{t}$ and $\vc{\ddot{x}}^{\text{e}}_{t}$ denote velocity and acceleration of the  end-effectors respectively.
% \begin{equation}
% 	L_{dx} = w_{dx} \lVert \vc{\Bar{\dot{x}}}^{\text{e}}_{t}- \vc{\dot{x}}^{\text{e}}_{t}\rVert^2
% \label{eq:temporal _loss_function}
% \end{equation}
% \begin{equation}
% 	L_{ddx} = w_{ddx} \lVert \vc{\Bar{\ddot{x}}}^{\text{e}}_{t}- \vc{\ddot{x}}^{\text{e}}_{t}\rVert^2
% \label{eq:orientation_loss_function}
% \end{equation}
% The primary goals and the secondary goals are distinguished by their weight terms. The weight term $w_{p}$
%  and $w_{ori}$ are set to $1000, 3600$ respectively while $w_{dx}$ and $w_{ddx}$ have value of $10$. This design strongly tract the result to satisfy the primary goals first. Then the mapper is slightly refined by the secondary goals.
%   \sehoon{need a bit more details}


\subsection{Mapping human motion to quadruped robot motion}
Conventional human-to-humanoid motion mapping framework has demonstrated solid and safe motion projection. \sehoon{citation} However, our mapping layer aims to create the human-to-quadruped robot motion mapping framework that shows high interactivity, the capability of a wide range of motion and the ability to demonstrate the semantics of the motion. To achieve these goals, we introduced the implicit representation based method used by the field of vision~\cite{Saito_2020_map} that is proficient in representing non-linear relationships even in unseen data regions.\sehoon{This technique is not clearly explained} Specifically, as a deep neural network(DNN) presents a high power for working as a complicated implicit function, we use the DNN layer working as an implicit mapping function.
\par
The key idea for composing the DNN layer as a mapper is learning from sparse motion pair samples. One motion pair sample consists of a triplet of the human posture and a triplet of the corresponding robot posture selected by the user. The user put the intention of mapping only by the posture selection that consequently reflected through the whole mapping relationship. For instance, the user can match the human locomotion pose to the robot locomotion. \sehoon{or not! That's the key} Preferentially, the user can pair the human arm manipulation pose to the robot front leg reaching pose. The trained DNN satisfies the selected sample motion relation while providing proper implicit mapping relation for unseen data. Using only sparse datasets brings the freedom of manual engineering that includes explicitly defining the posture relation, constraining joint limits and defining the corner cases. Furthermore, the learned mapper shows the capability of complicated and flexible full-mapping between completely different configured characters, a human and a quadruped robot. \sehoon{temporal/morphological inconsistency} In comparison to the optimization-based mapper, the DNN mapper operates in real-time.
\par
For composing a training data set, a user picks triplets of the human postures from the sampled short motion clips. We gather 10$\sim$20 short human motion clips for each task. An actor performs a simple motion of desired task motion captured by Microsoft's Azure Kinect. Taking a tilting motion as an example, an actor tilts the body along the roll axis to generate a single motion clip. Likewise, tilting along the pitch and yaw axis are sampled for the training tilting motion mapper. The human input features for the mappings are derived from two body orientations and eight points on a body. A hip orientation(root orientation) represents global information while a chest orientation relative to hip orientation symbolizes the local tilting status of the body. Eight key points are the 3D joint location of elbows, hands, knees and feet. The elbows and hands are represented relative to the shoulder position and the root orientation. The lengths of the points are normalized with a shoulder to wrist length. Similarly, knees and feet locations utilize the hip positions and hip to foot lengths for localization and normalization respectively. Corresponding robot pose triplets to the human pose triplets are sampled from the motion generator which is described specifically in the following subsection. \sehoon{This paragraph can be shortened}
\par
The simple pose-to-pose mapping has several limitations as ambiguity when mapping the cyclic motion or lack of ability to distinguish the moving feet. The reason is that a single posture can not handle a temporal factor. We augment the past two frames of the pose data constructing posture triplet to obtain temporal details to the network. The network implicitly processes the human pose history and explicitly calculate the loss function using the robot pose history. \sehoon{this should come earlier}
\par
We use multi-layer perceptron(MLP) for the mapping network. Our MLP consists  of three leaky ReLU layers and one final hyperbolic tangent layer. Since a hyperbolic tangent function outputs the value between [-1, 1],  we shift and scale the outputs using the robot joint limit vector to finalize the joint angle of the robot. The loss function primarily aims to minimize the joint pose and body orientation difference. Additionally, the loss function tries to minimize temporal components, global feet velocity and acceleration difference but with a lower priority. 
\begin{equation}
	L_{map}  = w_{q} \lVert \rVert^2 +  w_{dq} \lVert \rVert^2 + w_{ddq} \lVert \rVert^2 + w_{ori} \lVert \rVert^2 
\label{eq:mapping_loss_function}
\end{equation}
% Need to fill out the convention or nomenclature
The weight term $w_{q}$
 and $w_{ori}$ are much larger than $w_{dq}$ and $w_{ddq}$ for this design. \sehoon{need a bit more details}

% \subsection{Motion generator}
% We utilized the motion generators for two uses: generating robot motion for mapper training sets and providing reference motion for the reinforcement learning policy. Each motion generator is assigned to produce each task. The generating vector, $\vec{\alpha}$ which is also varied by the desired tasks decides the kinematic poses to generate. For example, the generating vector for tilting task $\vec{\alpha} = {a_{x}, a_{y}, a_{z}}$ which $a_{i}$ indicates the tilting angle for axis $i$. From decided $\vec{\alpha}$, the tilting motion generator solves the inverse kinematics(IK) to obtain the result robot pose. Likewise, the motion for each goal is determined by the generating vector. See the appendix for detailed generating vector formulation and motion generator function structure. The generated poses with noise injection are also used to feed for training the control policy. A detailed explanation related to it is written in the section V-A. \sehoon{merged with human data generation}

\subsection{Kinematic consistency mapping}
MLP implicit function outputs loose mapping without hard constraints or strict relation. This method offers a wide range of mapping with any human motion. However, the mapper often violates the kinematic plausibility of a result motion that leads RL policy learning to failure. \sehoon{in general, the description should provide a bit mathematical details.} \sehoon{should be faster than a regular IK...} 

\sunwoo{I just wrote below paragraphs}\par
\noindent \textbf{Contact consistency layer}
One of the most critical components of kinematic plausibility is contact consistency which we define as not moving and still in contact foot from the previous frame. The violation of contact consistency destabilizes the robot balancing, hence leading to learning failure.  Constraining the contact consistency with MLP loss function often fails to learn since the contact calculation requires the comparison operation that involves gradient vanishing. We propose an auxiliary layer that indicates the probability of contact consistency. The probability vector of contact consistency at time $t$, $\vc{c}_t$, indicates the contact consistent for leg $i$ if $c_{thr} > \vc{c}_t[i]$ and moving otherwise. The mapped pose is modified by dragging contact consistent feet to the location of the previous frame by solving IK. The resulting pose guarantees contact consistency with pose history while keeping the freedom of moving feet. The loss function $L_{cp}$ for training contact probability layer is defined as below:
\begin{multline}
	L_{cp}  = w_{cont} \lVert \text{CFH}(\vc{\Bar{p}}_{t}) -  \vc{c}_t \rVert^2 +  \\
	w_{mov} \lVert \text{CMV}(\vc{\Bar{p}}_{t-1:t}) -  \vc{c}_t \rVert^2
\label{eq:contact_consistency_loss_function}
\end{multline}
The first term of the loss function compares the loss with clipped foot height. The function $\text{CFH}$ stands for the clipped feet height function. It takes joint angles of the training data to calculate the feet height from the ground. Then, the function scale and clip the feet height to fit in a range of [-1, 1]. The function $\text{CMV}$ calculates the end-effector movement from given two frames of training data. It also fits the value to a range of [-1, 1].
\par
\noindent \textbf{Temporal consistency layer}
Sudden motion transition causes the kinematic violation, often causing the policy to perform a radical motion that falls into dangerous status. Guaranteeing temporal consistency prevents the sudden movement of the mapped motion, therefore, providing kinematic plausibility. We clipped the joint angle compared to the previous frame pose by joint velocity limit.  

\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{fig/SynthesizedMotionMapper.png}
\caption{Motion synthesis of tilting and manipulation task}
\end{figure}
\subsection{Motion Mapper Design for Complex Tasks}
The goal of our system is to provide smooth and solid robot control for any human motion input. Although every single mapper is trained separately, the overall mapper should produce a corresponding robot motion that can be a motion from a single mapper or a combination of motions from learned mappers. We introduce the state machine based mapping to handle this problem as shown in Figure XXX. The state machine consists of three mapping states and two neutral states depending on balance strategies. Three mapping states are standing, sitting, and walking. The standing state includes the tilting and one leg manipulation task which the balance strategy utilizes four legs to support the body in static circumstances. The robot tilts the body and freely manipulates the front legs in the sitting state. Unlike other states, walking involves a dynamic balancing that continuously adapts to the environment. The neutral states assist the smooth transition between states, forcing the programmed motions for the state transitions.
\par
Each mapping state consists of single or multiple motion mappers to form a single mapping motion. To synthesize a single mapping from multiple mappers, we build a hierarchy of mapping to decide the final posture. As a diagram of the standing state shown in Figure XXX, the tilting mapper builds the base motion. Using the contact consistency vector of the manipulation, the system determines a moving leg if it is present. The synthesizing layer then substitutes the selected leg to the manipulation motion. In the same way, each state has an assigned hierarchy of the mapping that decides the priority of the mapping pose.
\par
 When the state machine is on the transition between mapping states, the result motion doesn't show the mapped motion from the human motion. Instead, the mapping state goes to the neutral state to generate a smooth transition between mapping. The transition between neutral states is activated with programmed motion if it is needed. The transition detector takes the eight frames of human postures and the current mapping state for distinction. It detects key signals from the given human motion.
 \par 
The transition detector takes the eight frames of human postures and the current mapping state for distinction. It detects key signals from the given human motion. When the state machine is on the transition between mapping states, the result motion doesn't show the mapped motion from the human motion. Instead, the mapping state goes to the neutral state to generate a smooth transition between mapping. The transition between neutral states is activated with programmed motion if it is needed. This method has a disadvantage in agility when processing the transition but, it guarantees the smooth and solid transition from the mapping state to state.
